Sketch-GNN: Scalable Graph Neural Networks with Sublinear Training Complexity

Graph Neural Networks (GNNs) are widely applied to graph learning problems such as node classification. When scaling up the underlying graphs of GNNs to a larger size, we are forced to either train on the complete graph and keep the full graph adjacency and node embeddings in memory (which is often infeasible) or mini-batch sample the graph (which results in exponentially growing computational complexities with respect to the number of GNN layers). Various sampling-based and historical-embedding-based methods are proposed to avoid this exponential growth of complexities. However, none of these solutions eliminates the linear dependence on graph size. This paper proposes a sketch-based algorithm whose training time and memory grow sublinearly with respect to graph size by training GNNs atop a few compact sketches of graph adjacency and node embeddings. Based on polynomial tensor-sketch (PTS) theory, our framework provides a novel protocol for sketching non-linear activations and graph convolution matrices in GNNs, as opposed to existing methods that sketch linear weights or gradients in neural networks. In addition, we develop a locality-sensitive hashing (LSH) technique that can be trained to improve the quality of sketches. Experiments on large-graph benchmarks demonstrate the scalability and competitive performance of our Sketch-GNNs versus their full-size GNN counterparts.

==> old/background-old.tex <==
\section{Preliminaries of GNNs and Sketches}

\cm{Basic Notations.}
Consider a graph with $n$ nodes and $m$ edges. Connectivity is given by the adjacency matrix $A\in\{0,1\}^{n\times n}$ and features are defined on nodes by $X\in\sR^{n\times d}$ with $d$ the number of features. Given a matrix $C$, let $C_{i,j}$, $C_{i,:}$, and  $C_{:,j}$ denote its $(i,j)$-th entry, $i$-th row, $j$-th column, respectively. We use $\odot$ to denote the element-wise (Hadamard) product. And we use superscripts to refer to different copies of same kind of variable. For example, $X^{(l)}\in\sR^{n\times d_l}$ denotes node representations on layer $l$. 

\cm{Unified view of GNNs.}
A Graph Neural Network (GNN) layer takes the node representation of a previous layer $X^{(l)}$ as input and produces a new representation $X^{(l+1)}$, where $X=X^{(0)}$ is the input features.

Although GNNs are designed following different guiding principles, such as, neighborhood aggregation (GraphSAGE~\citep{hamilton2017inductive}, spatial convolution (GCN~\citep{kipf2016semi}), self-attention (GAT~\citep{velivckovic2017graph},  Weisfeiler-Lehman (WL) alignment (GIN~\citep{xu2018powerful}), etc, nearly all GNNs can be interpreted as performing message passing on node features, followed by feature transformation and an activation function. The update rules of GNNs can be typically written in the form
\begin{equation}
\label{eq:gnn}
X^{(l+1)} = \nonlinear\left(\sum_{s} C^{(s)}X^{(l)}W^{(l,s)}\right),
\end{equation}
where $C^{(s)}\in\sR^{n\times n}$ denotes the $s$-th convolution matrix that defines the message passing operator, $s\in\sZ_+$ denotes index of convolution, and $\nonlinear(\cdot)$ denotes the non-linearity. $W^{(l,s)}\in\sR^{d_l\times d_{l+1}}$ is the learnable linear weight matrix for the $l$-th layer and $s$-th filter. Within this common framework, GNNs differ from each other by choice of convolution matrices $C^{(s)}$, which can be either fixed (GCN, SAGE, GIN) or learnable (GAT). We re-formulate some popular GNNs into this framework; see~\cref{apd:gnns} for details. If not otherwise mentioned, we assume $s=1$ to simplify the notations. Learnable convolution matrix is only considered for GAT in~\cref{sec:alrogithm}, we assume the convolution matrix is fixed, e.g., $C=A$ for GCN, if not specifically noted.


\paragraph{Count Sketch and Tensor Sketch.} \emph{Count sketch}~\citep{charikar2002finding,weinberger2009feature} is an effective dimensionality reduction method which projects an $n$-dimensional vector $\vu$ into a smaller $c$-dimensional space through a random hash function $h:[n]\rightarrow [c]$ and a binary Rademacher variable $s:[n]\rightarrow \{\pm 1\}$, where $[n]=\{1,\cdots,n\}$, defined as $\countsketch{\vu}_i=\sum_{h(j)=i} s(j) \vu_j$. Count sketch of $\vu\in\sR^d$ is representable as a linear transformation $H\vu$. Here, $H\in\sR^{c\times n}$ is the so called \emph{count sketch matrix}. Count sketch transform on two vectors $\vu, \vv$ preserve the dot product, i.e., $\ip{\vu}{\vv}=\rmE\left[\ip{\countsketch{\vu}}{\countsketch{\vv}}\right]$.

\emph{Tensor sketch}~\citep{pham2013fast} is proposed as a generalization of count sketch to tensor product of vectors. Given $z\in\sR^n$ and a degree $k$, consider pair-wise independent hash functions $h_1,\cdots,h_k: [n]\rightarrow[c]$ and binary Rademacher variables $s_1,\cdots,s_k:[n]\rightarrow \{\pm 1\}$. Tensor sketch project $x$ into the $\sR^c$, defined as $\tensorsketch{k}{z}_i=\sum_{(h_j(j_1)+\cdots+h_k(j_k)) \bmod c=i} s_1(j_1)\cdots s_k(j_k)z_{j_1},\cdots,z_{j_k}$. Tensor sketch was used for approximating of the power of dot-product between vectors,i.e., it holds that $\left(\ip{\vu}{\vv}\right)^{(k)}=\rmE\left[\ip{\tensorsketch{k}{\vu}}{\tensorsketch{k}{\vv}}\right]$.
By definition, tensor sketch of degree $k=1$ falls back to count sketch, $\tensorsketch{1}{\cdot}=\countsketch{\cdot}$.

We define count sketch on a matrix $Z\in\mathbb{R}^{d\times n}$ as the count sketch of each row vector stacked, i.e., $\countsketch{X}\in\sR^{d\times c}$, and $\countsketch{Z}_{i,:}=\countsketch{Z_{i,:}}$. The same definition generalizes to tensor sketch, and~\citet{pham2013fast} devised a fast way to compute tensor sketch using the Fast Fourier Transform (FFT). Given $Z\in\sR^{d\times n}$, sketch dimension $c$ and degree $k$,
\begin{equation}
\label{eq:tensor-sketch}
\begin{split}
&\tensorsketch{k}{Z}=\mathrm{FFT}^{-1}\Big(\FFT{\mathrm{CountSketch}^{(1)}(Z)}\\
&\odot\cdots\odot\FFT{\mathrm{CountSketch}^{(k)}(Z)}\Big)
\end{split}
\end{equation}
where $\mathrm{CountSketch}^{(i)}(\cdot)$ denotes the count sketch with hash function $h_i$ and Rademacher variable $s_i$. $\FFT{\cdot}$ and $\IFFT{\cdot}$ are the Fast Fourier Transform and its inverse applied to each row of
a matrix, respectively.



==> old/introduction-old.tex <==
\section{Introduction}

Graph Neural Networks (GNNs) encompass state-of-the art methods for learning graph-based representations. They have been widely applied to various downstream tasks such as classification~\citep{scarselli2008graph,kipf2016semi}, clustering~\citep{bianchi2020spectral}, recommendation systems~\citep{wu2020graph}, social networks~\citep{fan2019graph}, etc. GNNs on graph data exploit the local / global information of the graph's structure to learn the representation of a target node through information aggregated from neighborhoods.

Since the invention of Graph Convolutional Networks (GCNs), numerous types of GNNs have be proposed to implement different design ideas such as message aggregations (GraphSAGE, PNA)~\citep{hamilton2017inductive,corso2020principal}, self-attention (GAT)~\cite{velivckovic2017graph}, and maximal expressiveness (GIN)~\citep{xu2018powerful}, among other schemes. However, the utilization of the graph topology makes it difficult to scale the learning to larger graphs or to deeper models with desirable computational and memory efficiency. Using a full-batch approach, which stores the Laplacian of the entire graph in memory, requires a memory complexity of $\mathcal{O}(ndL+d^2L)$ for an $n$-node graph with node features of dimension $d$ on an $L$-layer GCN. This linear memory complexity dependence on $n$ and the limited capacity of GPU memory restrict the training of large graphs with millions of nodes or more. As an example, the \textit{MAG240M-LSC} dataset~\citep{hu2021ogb} is a node classification benchmark with over 240 millon nodes, and requires over 202 GB memory when completely loaded. 

To address memory restrictions, several mini-batch sampling-based approaches have been proposed~\citep{hamilton2017inductive,chen2017stochastic,chen2018fastgcn}, with the idea of implementing message passing only between the neighbors contained with a sampled mini-batch, rather than the entire neighborhood. Another line of work addressing the memory restrictions is the historical-embedding based techniques (GNNAutoScale, VQ-GNN)~\citep{fey2021gnnautoscale,ding2021vq}, which maintain the expressive power of GNNs on mini-batch sampled subgraphs using some historical embeddings. However, all of the main stream methods relies on mini-batches. The number of mini-batches required is proportional to size of the graph, which significantly increases computational complexity for larger graphs in exchange for memory scalability. Although the memory bottleneck is avoided, we needs extremely long time to train a simple GNN on a large graph, for example, training a 4-layer GCN with just 333K parameters (1.3 MB) for 500 epochs on \textit{ogbn-papers100M} can take more than 2 days on a powerful AWS p4d.24x large instance~\citep{hu2021ogb}.

The community is still desperately looking for a principled method to efficiently train simple GNNs on large graphs, with both memory and time complexities sublinear or even independent to the graph size, at the expense of minimal loss of accuracy. This is actually not a daydream. Intuitively, the training of massage passing neural networks (MPNNs) traverse through the local neighborhoods on a graph, but probably we do not need to look at every of them before the weights converge, as there are many similar neighborhoods across a large graph. Moreover, widely-used GNNs are usually small and shallow with limited expressive power, indicating that a small proportion of data may be enough. 

This paper presents Sketch-GNNs, a framework to train GNNs with garph-size-independent scalability. Using the idea of sketching, which maps high-dimensional structures to a lower dimension through entry hashing, we sketch the $n\times n$ adjacency matrix, as well as the $n\times d$ node features before training. We derive the corresponding update rules on the sketches following the polynomial tensor sketch theory~\citep{han2020polynomial}, achieving graph size-independent memory and computational complexity during training, and the learned weights can be used by the standard models for inference. Moreover, we develop novel methods to learn and update the sketches of adjacency and features using learnable locality sensitive hashing (LSH)~\citep{chen2020mongoose}, which minimize the performance loss by adaptive increasing the sketch quality. This graph-size independent efficiency applies to not only GNNs with a fixed convolution matrix (GCN, GIN, GraphSAGE), but also to GNNs using changing convolution matrices (GAT).

To the best of our knowledge, our work is the first to use sketching techniques to make the training complexities sublinear to the data size, which is fundamentally different with the few existing work that sketch the weights or gradients of convolutional neural networks (CNNs) or fully-connected neural networks~\citep{kasiviswanathan2017deep,lin2019towards,spring2019compressing}. Our work is also the first to use learnable LSH technique to scale up GNNs, addressing the issues of the recent work that apply LSH for GNNs~\citep{kosman2021lsp,anonymous2022localitybased}.

==> rebuttal/comment_to_meta_reviewer.tex <==
Dear meta-reviewers, 

Thank you for your patience with moderating the reviewing process. We want to let you know that Reviewer #5 asked many questions about basic concepts and results which are clearly stated in the manuscript. For example, Reviewer #5 
(1) asked the definition of sketch ratio which is stated in multiple places (Line 223, Line 415, and the x-axis label of Figure 1), 
(2) asked about the sketch ratio used in Table 1 which is described in its caption, 
and (3) raised concerns that the information loss of sketching is not guaranteed, but Theorem 1 and 2 provide such results. 
Answers to superficial questions such as the ones mentioned above are not included in our response. 

Since most of these questions are about very fundamental and clearly stated components, it is questionable whether Reviewer #5 has spent enough time to read our paper and has a correct understanding of the proposed approach. 

To summarize, we think Reviewer #5 did not make a meaningful assessment of our paper and we kindly hope the meta-reviewers take this into consideration when making a fair judgment of our paper. Your understanding is very much appreciated.

Best regards,
Paper6934 Authors

==> rebuttal/long_version.tex <==

\category{Theory and Technical Questions}
%%%%%%%%%% R1A1 & R1A2 %%%%%%%%%%
\question{Dependence of sketch dimension $c$ in $n$.}{\reviewer{13}}
We agree that the sketch dimension $c$ has to be an increasing function of the graph size $n$ to keep the error bounded, but $c$ does not have to be proportional to $n$ to achieve good performance (in Tab.3 a smaller sketch ratio $c/n$ is adequate on a larger graph). We originally described this as ``graph size-independent scalability'' to reflect that $c$ can be chosen based on the performance required. However, we agree this term may cause confusion and we will change it to ``sublinear scalability''.
In practice the sketch ratio $c/n$ required to maintain similar performance as the ``full-graph'' model is decreasing. In Tab.3, $c/n=0.4$ is needed on \textit{ogbn-arxiv} with 169K nodes but $c/n=0.2$ is adequate on \textit{ogbn-product} of size 2.45M. When setting $c$ to be a constant, the performance is decreasing (compared w.r.t. the ``full-graph'' baseline) when $n$ is increasing.
%%%%%%%%%% R3A1 %%%%%%%%%%
\question{Dependence of \#sketches $r$ in $n$.}{\reviewer{3}} 
Form Thm.2, we need $r=\sqrt[j]{n}$ sketches for some $j\ge1$ s.t. $c\ge(2+3^j)/(\epsilon^2\delta)$. Thus, for fixed $\epsilon$ and $\delta$, we have $j=O(\log_3 c)$ and $r=\Omega(3^{\log_c n})$. If $n$ is not too small, $\log_c n\approx1$ and the dependence of $r$ in $n$ is negligible. We find setting $r=3$ is enough in the experiments. We will expand these discussions with more details in the appendix to give the readers a clearer understanding of the complexity dependencies.
%%%%%%%%%% R3A4 %%%%%%%%%%
\question{Dependence of the sample size $|B|$ in $n$.}{\reviewer{3}}
Because of the ``slow change'' phenomenon of the data-dependent hash tables (left sub-figure of Fig.2), we do not expect large updates of the LSH functions after the early phase of training, and we only need a small subset of nodes whose hash codes are likely outdated to update the LSH functions. As described in part (1) of challenge (2) in Sec.4, we select a constant number of hash buckets with the largest gradients and thus $|B|=O(n/c)$ which increases slowly w.r.t. $n$. We will make this point clearer in Sec.4.
%%%%%%%%%% R3A6 %%%%%%%%%%
\question{Data-independence and uniformity assumptions of hash functions.}{\reviewer{3}}
Actually without data-independence and uniformity assumptions of the hash functions, similar concentration bounds can still be established (e.g., Thm.3 in~\citep{weinberger2009feature}), and the corresponding algorithm is known as feature hashing. Feature hashing is essentially identical to count sketch but usually with data-dependent hash functions and mean estimator. Intuitively, it is more challenging to bound the collision errors with randomized hash functions and the median estimator is introduced as it is more robust (Sec.3.2 of~\citep{charikar2002finding}). The sketches in Sketch GNN are learned using gradient descent and thus it is hard to obtain an error bound. Thus we build upon count and tensor sketch theory and obtain an error bound when relaxed to randomized hashing. We will discuss about feature hashing and some alternative sketching error bounds (e.g.,~\citep{meister2019tight}) in the appendix.
%%%%%%%%%% R3A2 %%%%%%%%%%
\question{Error bound in the sense of expectation.}{\reviewer{3}}
Indeed, Thm.1 is established in the sense of expectation. But we cannot train Sketch GNNs over different sketches per iteration, since the randomness in the sketches can impede training. Instead, the learnable LSH and sketches are introduced to compensate the fixed number of sketches. Thanks to the gradient signals, we are able to optimize the estimation over a fixed number of sketches directly. Proving an error bound on this learned estimation is much harder, so we relax to randomized sketches in Thm.1.
%%%%%%%%%% R3A3 & R1A6 %%%%%%%%%%
\question{Sparsity of sketched adjacency.}{\reviewer{13}}
We did not assume the same sparsity after sketching, but actually, the (two-sided) count sketch of the convolution matrix, $\countsketch(\countsketch(C)\tran)\in\mathbb{R}^{c\times c}$ maintains some-level of sparsity if the convolution matrix $C$ is sparse. Recall that $\countsketch(\countsketch(C)\tran)=RCR\tran$, where $R\in\mathbb{R}^{c\times n}$ is the count sketch matrix which has only one non-zero entry per column (see Sec.2). If $C$ has at most $s$ non-zero entries per column (e.g., $s=d_\textrm{max}+1$ in GCN, where $d_\textrm{max}$ is the maximum node degree) and $c \gg s$ (usually holds in practice), it is not hard to find that there are at most $s$ non-zero entries per column in the product $RC\in\mathbb{R}^{c\times n}$. We can show $\countsketch(\countsketch(C)\tran)$, as a product of three highly sparse matrices, is still sparse. Thus, by using a sparse encoding of the sketch, we can avoid the $O(c^2)$ memory complexity term and be strictly $O(c)$.
%%%%%%%%%% R1A7 %%%%%%%%%%
\question{Learning polynomial coefficients $\{c_k\}$.}{\reviewer{1}}
In Sketch-GNN, we train the coefficients $\{c_k\}$ to optimize the classification loss of node classification directly. That is, we learn a set of polynomial activations in the same manner as we learn the other parameters. It is not that important whether the learned polynomial activations still approximate some known functions, as long as a good performance can be obtained. (The setup in Fig.1 is different, where we train $\{c_k\}$ to minimize the error w.r.t. the sigmoid activated embedding directly.)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Experiments and Additional Results}
%%%%%%%%%% R1A3 %%%%%%%%%%
\question{Goal of Sketch GNN and comparison with SGC.}{\reviewer{1}}
The goal of Sketch GNN is to approximate existing GNNs and achieve similar performance as the corresponding full-graph baseline with just sublinear training time and memory complexities. In practice, SGC and other simplified GNNs may achieve good performance on some datasets (e.g., $94.9$ F1 score on \textit{Reddit}), but there is no guarantee that their performance is always close to multi-layer GNNs'. Moreover, although SGC is memory efficient in the sense that only the pre-computed embedding and one weight matrix are needed, the memory complexity is still linear in $n$. On \textit{Reddit}, Sketch GraphSAGE with sketch ratio $c/n=0.3$ can also achieve $94.85\pm0.61$ F1 score (Tab.1) with 1686 MB memory usage (slightly larger than SGC's 1519 MB). Although the performance and efficiency are similar to SGC's on \textit{Reddit}, we expect Sketch GNNs to work better on more datasets (due to the error guarantee) and scale better on larger graphs (due to the sublinear complexities). We will add the SGC baseline to Sec.7.
%%%%%%%%%% R1A4 %%%%%%%%%%
\question{Ablation studies with fixed sketches.}{\reviewer{1}}
The Sketch-GCN with learned sketches and ratio $c/n=0.2$ can achieve $0.7004\pm0.0096$ on \textit{ogbn-arxiv}. However, the same model with fixed randomized sketches can only achieve $0.6649\pm0.0106$. These performance gaps can be observed on other models datasets and address the necessity of the LSH-based sketch. We will add the corresponding ablation studies to the appendix.
%%%%%%%%%% R3A10 %%%%%%%%%%
\question{Comparison of convergence time.}{\reviewer{3}}
We agree that convergence time could be a better metric to compare Sketch GNN with sampling-based methods. We define the ``convergence time'' as the time for the validation accuracy to reach $99\%$ of the best and find that on \textit{ogbn-arxiv} with sketch dimension or mini-batch size set to $0.1n$ (the setup in Tab.1), the convergence time of Sketch GCN is $88\pm8$ s, slightly better than VQ-GNN's ($103\pm11$ s) and GraphSAINT's ($120\pm4$ s). Sketch GCN takes longer number of epochs to converge, but the convergence time is smaller because of the shorter time per epoch. We will add more results and discussions to the appendix.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Clarifications and Other Questions}
%%%%%%%%%% R3A5 %%%%%%%%%%
\question{Experiments not showing value of Sketch GNN?}{\reviewer{3}}
We do not agree with these arguments. Firstly, we already test Sketch GNN on \textit{ogbn-product} with 2.45M nodes which is larger than most other graphs. Secondly, with appropriate sketch ratios ($0.2 \sim 0.4$ in Tab.3) the performance is always competitive w.r.t. the baselines. It is only when we use a small sketch ratio $0.1$ on a small dataset \textit{ogbn-arxiv} the performance is slightly affected (Tab.2), and under this setup only 38.7 MB memory is used (Tab.1), far less than the device limit. The reduction in epoch time is considerable (Tab.1), since we usually train GNNs for hundreds of epochs. For example, when training for 500 epochs, Sketch GCN will be 181 s faster than full-graph GCN and 85 s faster than GraphSAINT GCN, which are much larger than the pre-processing overhead 27 s. Furthermore, the implementation of sketching (pre-processing) algorithm is not optimized. We expect further speed up if using a sparse FFT algorithm instead of standard FFT. Detailed discussion on the implementation issues will be added to the appendix.
%%%%%%%%%% R5A1 %%%%%%%%%%
\question{Sketching is not efficient?}{\reviewer{5}}
We believe sketching is efficient because: (1) it is an one-time cost, and (2) count and tensor sketch can implemented by sparse matrix multiplication and Fast Fourier Transform, which are supported by highly-optimized libraries like PyTorch. Moreover, the time complexity of count and tensor sketch is better than the other Johnson Lindenstrauss transforms~\citep{meister2019tight}.
%%%%%%%%%% R5A2 %%%%%%%%%%
\question{Information loss of sketching is not clear?}{\reviewer{5}}
In theory, we approximate the original update rule of a GNN With sketching, and the approximation errors are bounded (Thm.1\&2). In practice, we can achieve competitive performance on \textit{ogbn-product} with 2.45M nodes with a $0.2$ sketch ratio.
%%%%%%%%%% R5A4 & R5A5 %%%%%%%%%%
\question{Definitions of sketch and compression ratio.}{\reviewer{5}}
The sketch ratio is defined as $c/n$, the sketch dimension $c$ over the input dimension $n$, in multiple places in the paper (L.223, L.415, and the x-axis label of Fig.1). We use ``compression ratio'' in Tab.2 because we are comparing with the graph coarsening algorithm, which is a ``pre-compression'' algorithm as ours. Compress ratio, as its name suggests, is the ratio between the uncompressed size and the compressed size. For Sketch GNN, compress ratio is slightly larger than sketch ratio, since there are some memory overheads for learnable LSH. We will add more details on this to Sec.7. The sketch ratio used in Tab.1 is $0.1$ (stated in the caption of Tab.1). The training time complexity of Sketch GNN is $O(c)$.
%%%%%%%%%% R5A6 %%%%%%%%%%
\question{Tab.1 and Tab.2\&3 under different settings?}{\reviewer{5}}
Tab.1 is for the comparison of efficiency while Tab.2\&3 are for performance. The performance of the experiments in Tab.1 on \textit{ogbn-arxiv} can be found in Tab.2\&3. We will add more performance results on \textit{Reddit} to the appendix.
%%%%%%%%%% R3A11 %%%%%%%%%%
\question{Baseline performance lower than leaderboard's?}{\reviewer{3}}
The listed performance of full-graph GCN, full-graph GraphSAGE, and VQ-GNN in Tab.2\&3 are copied from the OGB leaderboard or original paper. The other results (full-graph GAT, GraphSAINT, Graph Coarsening) could be slightly lower than the elsewhere reported because we only run 500 epochs and repeat the experiment for 5 times. In general these slight differences are within the error bars.
%%%%%%%%%% R3A7 %%%%%%%%%%
\question{Learnable parameters in learnable LSH.}{\reviewer{3}}
The projection matrix $P$ in Eq.3 is exactly what we learn in the learnable LSH algorithm as originally proposed in the Sec.3.3.1 of~\citep{chen2020mongoose}. The SimHash algorithm described in Sec.2 is the standard non-learnable version. We will refine the corresponding part in Sec.4.
%%%%%%%%%% R3A9 %%%%%%%%%%
\question{Relation to graph homophily.}{\reviewer{3}}
LSH does not depend on the topology of the graph, i.e., whether we put two nodes in the same bucket has noting to do with their adjacency. Sketch GNN does not make any assumptions on the homophily and should work equally well for low- and high-homophily graphs.
%%%%%%%%%% R3A8 %%%%%%%%%%
\question{How to hash correctly with online learned LSH?}{\reviewer{3}}
This is exactly the second challenge described in Sec.4. See Challenge (2) for details and the right sub-figure of Fig.2 for the proof-of-concept experiments.
%%%%%%%%%% R5A2 %%%%%%%%%%
\question{Why $O(ncd)$ overhead of SimHash in L.242?}{\reviewer{5}}
SimHash on each feature vector (Eq.3) requires $O(cd)$ time and memory and we have $n$ of them. Hence the total time overhead introduced is $O(ncd)$.
%%%%%%%%%% R1A5 %%%%%%%%%%
\question{Straight-forward sub-simple approach?}{\reviewer{1}}
We are not sure if we correctly understand this question. If the approach mentioned is the neighbor sampling algorithm which train GNN on a batch of local neighborhoods (i.e., ego-graphs if direct neighborhood), we have considered GraphSAINT as a baseline of mini-batch sampling methods. In GraphSAINT, GNNs are trained on a batch of local sub-graphs and the memory scalability issue is solved. However, Sketch-GNN is faster than GraphSAINT as we only need to train on the sketched input (sub-linear time complexity) instead of traversing the large graph (see Tab.1). Please correct us and point to the reference/implementation if you meant to refer to some other algorithm.
%%%%%%%%%% R1A8 %%%%%%%%%%
\question{Missing details about sparse froward-pass.}{\reviewer{1}}
The technique used in the final layer of Sketch-GNN is identical to the Algorithm 1 in~\citep{chen2020slide}. We will add the detailed description of the sparse forward-pass and back-propagation algorithm in Sec.3.1 of~\citep{chen2020slide} to our appendix to be self-consistent. 
%%%%%%%%%% R1A11 & R3A12 %%%%%%%%%%
\question{Suggested citations.}{\reviewer{13}}
\citep{yang2019nodesketch} produce graph embeddings as recursive sketches of the adjacency matrix, which preserve the high-order node proximity. In our work, the single-sided sketches of the convolution matrix $\countsketch(C)\tran\in\mathbb{R}^{n \times c}$ can also be thought as node embeddings, but we use the two-sided sketches $\countsketch(\countsketch(C)\tran)$ as a generalized form of adjacency in Sketch-GNNs. \citep{sato2022constant} provides theoretical guarantees to estimate the node embeddings in MPNNs under the uniform node sampling scheme with constant time per node (thus still proportional to $n$ per epoch). \citep{zeng2021decoupling} propose a novel way to apply GNNs on sampled subgraphs, which decouple the depth and scope of GNNs and lead to better expressivity and scalability. We are interested to add new advances on graph sampling like this to the related work discussion, and consider it as a baseline in the added experiments. We are going to discuss these lines of research in detail in the appendix. 
%%%%%%%%%% R1A9 & R1A10 %%%%%%%%%%
\question{Correcting citations and margins.}{\reviewer{1}}
We have done a throughout check of the bibliography list and correct these problems. We have corrected all the margin sizes.
%%%%%%%%%% R5A7 %%%%%%%%%%
\question{Why separating Sec.3\&4?}{\reviewer{5}}
We separate Sec.3 (polynomial tensor sketch) and Sec.4 (learning sketches with LSH) because (1) they are two main components of Sketch GNN, and (2) they are orthogonal in the sense that the former answers how to compress GNNs and approximate the original update rules with sketches, while the latter addresses how to learn and update the sketches.
%%%%%%%%%% R5A8 %%%%%%%%%%
\question{More than sufficient discussions?}{\reviewer{5}}
We believe Sec.3\&4 are necessary, since they address two major components of Sketch GNN. We will rewrite Sec.4 to improve the presentation. We plan to move Sec.5 (generalizing to other GNNs) to the appendix. We will expand Sec.7 with the added results and ablation studies.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> rebuttal/main_response.tex <==

\textbf{Paper6934-SketchGNN.} We thank all reviewers for their valuable feedback. We are glad the reviewers consider our approach novel~\reviewer{135}, theory~\reviewer{15} and evaluations~\reviewer{1} sound, presentation clear~\reviewer{3}. They agree that our paper brings new perspective~\reviewer{35} and significant contributions~\reviewer{15} to the GNN community. We will modify our paper as suggested such as rewording \textit{graph-size independent} to \textit{sublinear}, and adding suggested citations, baselines and ablation studies. Below we address all concerns and present additional experiment results as requested.
%%%%%%%%%%
\question{``Graph-size Independent'' Scalability.}{\reviewer{13}}
We will reword the phrase to \textit{sublinear} to avoid confusion. Here, we clarify the following :%
\point{1}{Dependence of sketch dimension~$\bm{c}$ on graph size~$\bm{n}$}{\reviewer{13}.}
Training memory/compute cost does not depend on~$n$, excluding the one-time cost to calculate the sketches before training. Count/tensor sketch can be implemented via highly-parallel sparse-dense matrix multiplication and FFT, therefore \mention{sketching is efficient}{\reviewer{5}}. With sketching, we bound approximation errors (Thm.~1\&2), therefore \mention{the information loss of sketching is theoretically guaranteed}{\reviewer{5}}. Although the theoretical approximation error increases under smaller sketch ratio~$c/n$, we observe competitive experimental results with smaller~$c/n$ especially on large graphs. In practice, the sketch-ratio required to maintain ``full-graph'' model performance decreases with~$n$, as verified in Tab.~3:~$c/n=0.4$ is needed on \textit{ogbn-arxiv} with 169K nodes but~$c/n=0.2$ is adequate on \textit{ogbn-product} with 2.45M nodes.%
\point{2}{Dependence of \# of sketches~$\bm{r}$ on~$\bm{n}$}{\reviewer{3}.}
If~$n$ is not too small, the dependence of~$r$ on~$n$ is negligible: according to Thm.~2, for fixed approximation error~$\epsilon$ and probability~$\delta$, we need~$r=\Omega(3^{\log_c n})$ sketches. In all experiments,~$r=3$ achieves SOTA results.%
\point{3}{Dependence of sample size~$\bm{|B|}$ on~$\bm{n}$}{\reviewer{3}.}
$|B|$ increases slowly w.r.t.~$n$ since we select a constant number of hash buckets with the largest gradients, due to the ``slow change'' phenomenon of the data-dependent hash tables (Fig.~2 left).%
%%%%%%%%%%
\question{$\bm{O(c)}$ Complexities and Sparsity of Sketches.}{\reviewer{13}}
The two-sided sketch~$\countsketch(\countsketch(C)\tran)\in\mathbb{R}^{c\times c}$ maintains sparsity for sparse convolution~$C$, as~$\countsketch(\countsketch(C)\tran)=RCR\tran$ (a product of 3 sparse matrices) is still sparse, where count-sketch matrix~$R\in\mathbb{R}^{c\times n}$ has one non-zero entry per column. If~$C$ has at most~$s$ non-zeros per column, there are~$\le s$ non-zeros per column in~$RC$ when~$c\gg s$ (holds in practice). Thus, we avoid the~$O(c^2)$ memory cost and are strictly~$O(c)$.
%%%%%%%%%%
\question{Concerns about Theoretical Assumptions.}{\reviewer{13}}
We clarify our set of theoretical assumptions may not perfectly match reality because of the learnable LSH.
\marker{1} Without the \mention{data-independence and uniformity of hashing}{\reviewer{3}}, similar concentration bounds can still be established (Thm.~3 in ``Feature hashing for large scale multitask learning'', Weinberger et al.), and it is known as \textit{feature hashing}.%
\point{2}{The polynomial coefficients~$\bm{\{c_k\}}$}{\reviewer{1}} are learned to optimize the classification loss directly. The coeffs that obtain the best performance in experiments do not necessarily approximate a known activation. We defer the challenging problem of bounding the error of sketches and coeffs learned using gradients to future studies.%
\marker{3} Although the \mention{error bound is in expectation}{\reviewer{3}}, we do not train over different sketches per iteration, since the randomness causes instabilities. Instead, we introduce learnable LSH to counteract the approximation limitations caused by the fixed \# of sketches.%
%%%%%%%%%%
\question{Goal and Practical Value of SketchGNN}{\reviewer{13}}
\marker{1} The \mention{goal}{\reviewer{1}} of SketchGNN is to approximate existing GNNs and achieve performance similar to the corresponding full-graph baseline with sublinear training time and memory. We observe that learning the coefficient $\{c_k\}$ may further improve performance and evaluating the approximation errors is not crucial in practice. We will present the approximation results in the appendix.%
\point{2}{Size of graph evaluated is not large}{\reviewer{3}?}
We obtain competitive performance on \textit{ogbn-product} with 2.45M nodes (2nd largest node-classification benchmark in OGB).%
\point{3}{Reduction in time not significant}{\reviewer{3}?}
SketchGCN on \textit{ogbn-arxiv} is 72\% and 55\% faster than the corresponding full-graph and GraphSAINT baselines (Tab.~1), while the pre-processing time is just 14\% of overall reduction (running 500 epochs).%
%%%%%%%%%%
\question{Comparison with SGC.}{\reviewer{1}}
On \textit{Reddit}, Sketch-GNN with~$c/n=0.3$ achieves a comparable~94.85\textpm0.61 F1. Although SGC is efficient, the memory cost is still~$O(n)$ and there is no guarantee on its performance. SketchGNN has an error guarantee and a sublinear cost, verifying that it may perform better on more complex and larger datasets.%
%%%%%%%%%%
\question{Ablation Studies with Fixed Sketches.}{\reviewer{1}}
Learned sketches improve the performance for all models and datasets. Under~$c/n$=$0.2$, the Sketch-GCN with learned sketches achieves 0.7004\textpm0.0096 accuracy on \textit{ogbn-arxiv} while fixed randomized sketches achieve 0.6649\textpm0.0106.%
%%%%%%%%%%
\question{Comparison of Convergence Time.}{\reviewer{3}}
The wall-clock time for the validation accuracy to reach 99\% of the best accuracy is 88\textpm8s for SketchGCN, better than VQ-GNN's 103\textpm11s and GraphSAINT's 120\textpm4s, under setup of Tab.~1. We agree converge time is a nice metric to add.%
%%%%%%%%%%
\question{Other Issues.}{\reviewer{35}}
\point{1}{Baseline performance lower than leaderboard}{\reviewer{3}}
The listed performance of full-graph GCN, GraphSAGE, and VQ-GNN are copied from literature. The other results may be slightly lower because we have to keep the model sizes around the same and cannot tune the architectures.%
\point{2}{Learnable params in learnable LSH}{\reviewer{3}.}
The projection matrix~$P$ in Eq.~(3) is what we learn.%
\marker{3} LSH does not depend on graph topology, so SketchGNN should work equally well for \mention{low- and high-homophily graphs}{\reviewer{3}}.%
\point{4}{How to hash correctly with online learned LSH}{\reviewer{3}?}
This is described in challenge (2) of Sec.~4 and is experimentally verified (Fig.~2 right).%
\point{5}{Tab.~1 and Tab.~2\&3 under different settings}{\reviewer{5}?}
The performance of the experiments in Tab.~1 on \textit{ogbn-arxiv} can be found in Tab.~2.%

==> rebuttal/question_answer_list.tex <==
% QA COLORING
\definecolor{todo}{HTML}{BF00FF}
\definecolor{question}{HTML}{CC0000}
\definecolor{answer}{HTML}{333399}


\newtoggle{tcolor}
\newcommand{\choosecolor}{%
\iftoggle{tcolor}%
{\color{\colorone}\togglefalse{tcolor}}%
{\color{\colortwo}\toggletrue{tcolor}}%
}
\pretocmd{\item}{\choosecolor}{}{}

\def\colorone{question}
\def\colortwo{answer}

% BEGINNING OF LIST
\section{R1}

\begin{itemize}
    \item Q1: Theorem 1 tells that unless $c \to \infty$, the relative error may blow up as $n \to \infty$. To avoid the error blowing up, we need to set $c$ to be proportional to $n$, resulting in linear time complexity (or at least an increasing function w.r.t. $n$). A true constant time method would not blow up the error as $n \to \infty$ keeping the time consumption. I feel the claim of "Graph Size-Independent Scalability" may be an overclaim in this regard. It would be beneficial to discuss this point in detail.
    \item A1: We agree that the sketch dimension $c$ has to be an increasing function of the graph size $n$ to keep the error bounded, but $c$ does not have to be proportional to $n$ to achieve good performance (in Table 3 a smaller sketch ratio $c/n$ is adequate on a larger graph). We originally described this as ``graph size-independent scalability'' to reflect that $c$ can be chosen based on the performance required. However, we agree this term may cause confusion and we will change it to ``sublinear scalability''.
    
    \item Q2: In addition, in the experiments, $c$ seems an increasing function w.r.t. $n$ (though the ratio decreases.) How fast is the empirical growth rate? How the performance is affected if we set $c$ to be a constant as $n$ increases.
    \item A2: In practice the sketch ratio $c/n$ required to maintain similar performance as the ``full-graph'' model is decreasing. In Table 3, $c/n=0.4$ is needed on \textit{ogbn-arxiv} with 169K nodes but $c/n=0.2$ is adequate on \textit{ogbn-product} of size 2.45M. When setting $c$ to be a constant, the performance is decreasing (compared w.r.t. the ``full-graph'' baseline) when $n$ is increasing.
    
    \item Q3: I could not find the goal of this paper is whether efficiently approximating existing GNNs or efficiently achieving good performance in graph learning tasks. If the former is the case, the approximation errors should be evaluated in detail. If the latter is the case, there are many strong baselines such as SGC [1]. SGC achieves $94.9$ F1 on Reddit and seems much faster than the proposed method. The proposed method keeps nonlinearity using the polynomial tensor sketch unlike SGC, but it would be important to discuss this is worth maintaining for downstream tasks. ([1] Wu et al. Simplifying Graph Convolutional Networks. ICML 2019. https://arxiv.org/abs/1902.07153.)
    \item A3: The goal of Sketch GNN is to approximate existing GNNs and achieve similar performance as the corresponding full-graph baseline with just sublinear training time and memory complexities. In practice, SGC and other simplified GNNs may achieve good performance on some datasets (e.g., $94.9$ F1 score on \textit{Reddit}), but there is no guarantee that their performance is always close to multi-layer GNNs'. Moreover, although SGC is memory efficient in the sense that only the pre-computed embedding and one weight matrix are needed, the memory complexity is still linear in $n$. On \textit{Reddit}, Sketch GraphSAGE with sketch ratio $c/n=0.3$ can also achieve $94.85\pm0.61$ F1 score (Table 1) with 1686 MB memory usage (slightly larger than SGC's 1519 MB). Although the performance and efficiency are similar to SGC's on \textit{Reddit}, we expect Sketch GNNs to work better on more datasets (due to the error guarantee) and scale better on larger graphs (due to the sublinear complexities). We will add the SGC baseline to Section 7.
    
    \item Q4: The importance of learning sketches (Section 4) is not so convincing as the randomized one already ensures the approximation. It would be beneficial to conduct ablation studies in the experiments.
    \item A4: Thanks for the constructive advise. The Sketch-GCN with learned sketches and ratio $c/n=0.2$ can achieve $0.7004\pm0.0096$ on \textit{ogbn-arxiv}. However, the same model with fixed randomized sketches can only achieve $0.6649\pm0.0106$. These performance gaps can be observed on other models datasets and address the necessity of the LSH-based sketch. We will add the corresponding ablation studies to the appendix.
    
    \item Q5: A straightforward method to make an inductive GNN sublinear time is to sub-sample training data. As we can see the training data for GNN as a batch of ego-graphs, we do not need to use the entire graph (especially if the input graph is massive) from a practical point of view. It would be beneficial to compare the proposed method with such a naive approach in the experiments to highlight the effectiveness.
    \item A5: Thanks for the insightful question. We are not sure if we correctly understand this question. If the approach mentioned is the neighbor sampling algorithm which train GNN on a batch of local neighborhoods (i.e., ego-graphs if direct neighborhood), we have considered GraphSAINT as a baseline of mini-batch sampling methods. In GraphSAINT, GNNs are trained on a batch of local sub-graphs and the memory scalability issue is solved. However, Sketch-GNN is faster than GraphSAINT as we only need to train on the sketched input (sub-linear time complexity) instead of traversing the large graph (see Table 1). Please correct us and point to the reference/implementation if you meant to refer to some other algorithm.
    
    \item Q6: "Compact graph-size independent sketches (i.e., $O(c)$)" (L. 185 right) are a bit misleading because there is a hidden factor $m/n$, which depends on the input size in dense graphs, and the sketch size becomes $O(c^2)$ to absorb the factor.
    \item A6: Actually, the (two-sided) count sketch of the convolution matrix, $\countsketch(\countsketch(C)\tran)\in\mathbb{R}^{c\times c}$ maintains some-level of sparsity if the convolution matrix $C$ is sparse. Recall that $\countsketch(\countsketch(C)\tran)=RCR\tran$, where $R\in\mathbb{R}^{c\times n}$ is the count sketch matrix which has only one non-zero entry per column (see Section 2). If $C$ has at most $s$ non-zero entries per column (e.g., $s=d_\textrm{max}+1$ in GCN, where $d_\textrm{max}$ is the maximum node degree) and $c \gg s$ (usually holds in practice), it is nor hard to find that there are at most $s$ non-zero entries per column in the product $RC\in\mathbb{R}^{c\times n}$. We can show $\countsketch(\countsketch(C)\tran)$, as a product of three highly sparse matrices, is still sparse. Thus, by using a sparse encoding of the sketch, we can avoid the $O(c^2)$ memory complexity term and be strictly $O(c)$.
    
    \item Q7: I could not find how $c_k$ of the polynomial tensor sketch is trained (in Figure 1 and in Section 7.) Is it trained to optimize the approximation loss of the true activation or to optimize the classification loss of the downstream task? If the former is the case, how can we calculate the ground-truth value (without unsketching)? If the latter is the case, the resulting activation seems not to converge to the sigmoid function.
    \item In Sketch-GNN, we train the coefficients $c_k$ to optimize the classification loss of node classification directly. That is, we learn a set of polynomial activations in the same manner as we learn the other parameters. It is not that important whether the learned polynomial activations still approximate some known functions, as long as a good performance can be obtained. (The setup in Figure 1 is different, where we train $c_k$ to minimize the error w.r.t. the sigmoid activated embedding directly.)
    
    \item Q8: L. 201 claims "This technique is introduced in (Chen et al., 2020b) and is called sparse forward-pass and back-propagation. We describe the algorithm in detail in Section 4," but I could not find the corresponding descriptions in Section 4.
    \item A8: Sorry for the confusion. The technique used in the final layer of Sketch-GNN is identical to the Algorithm 1 in~\citep{chen2020slide}. We will add the detailed description of the sparse forward-pass and back-propagation algorithm in Section 3.1 of~\citep{chen2020slide} to our appendix to be self-consistent.
    
    \item Q9: The bibliography contains many published papers, but the arXiv versions are cited. For example, Andoni et al. "Practical and optimal lsh for angular distance" was published in NeurIPS, and Chen et al. "Stochastic training of graph convolutional networks with variance reduction" was published in ICML. Please update the bibliography information in the camera-ready.
    \item A9: Thanks for the carefulness. We have done a throughout check of the bibliography list and correct these problems.
    
    \item Q10: The margins below the section titles look reduced. Please follow the official style file and use the appropriate margins.
    \item A10: Thanks for help checking the style. We have corrected all the margin sizes.
    
    \item Q11: The literature is well cited. I have some suggestions for improvement. [1] applies sketching to adjacency matrices. Although the scope of [1] is not GNN, it would be important to point out the connection. [2] proposes constant time GNNs. Although the scope of [2] is not a per-epoch constant time algorithm, the complexities discussed in the related work section of the submission can be updated, especially in the dense case. ([1] NodeSketch: Highly-Efficient Graph Embeddings via Recursive Sketching. KDD 2019. https://dl.acm.org/doi/10.1145/3292500.3330951. [2] Constant Time Graph Neural Networks. TKDD 2022. https://arxiv.org/abs/1901.07868.)
    \item A11: Thanks for pointing us to these relevant work. \citet{yang2019nodesketch} produce graph embeddings as recursive sketches of the adjacency matrix, which preserve the high-order node proximity. In our work, the single-sided sketches of the convolution matrix $\countsketch(C)\tran\in\mathbb{R}^{n \times c}$ can also be thought as node embeddings, but we use the two-sided sketches $\countsketch(\countsketch(C)\tran)$ as a generalized form of adjacency in Sketch-GNNs. \citet{sato2022constant} provides theoretical guarantees to estimate the node embeddings in MPNNs under the uniform node sampling scheme with constant time per node (thus still proportional to $n$ per epoch). We are going to discuss these lines of research in detail in the appendix.
    
\end{itemize}


\section{R3}

\begin{itemize}
    \item Q1: For theoretical analysis, my biggest concern is that the "graph size-independent scalability" seems to be an overclaim. There are some "hidden" components in the algorithm that may inevitably introduce the $O(n)$ factor into the complexity. Specifically: To achieve the error bound of Theorem 1 (and Theorem 2), the number of hash functions and the sketch dimension $c$ will depend on the graph size $n$. This is stated in the proof in the Appendix (page 12, above Equation 8).
    \item A1: (Same as R1 A1) ... Form Theorem 2, we need $r=\sqrt[j]{n}$ sketches for some $j\ge1$ s.t. $c\ge(2+3^j)/(\epsilon^2\delta)$. Thus, for fixed $\epsilon$ and $\delta$, we have $j=O(\log_3 c)$ and $r=\Omega(3^{\log_c n})$. If $n$ is not too small, $\log_c n\approx1$ and the dependence of $r$ in $n$ is negligible. We find setting $r=3$ is enough in the experiments. We will expand these discussions with more details in the appendix to give the readers a clearer understanding of the complexity dependencies. 
    
    \item Q2: The error bound of Theorem 1 is in the sense of expectation. This means a "true" Sketch GNN training algorithm should generate a new sketch of the graph adjacency matrices and node feature matrices for every training iteration. So the proposed "preprocessing" in Algorithm 1 will break the error bound. Even though Algorithm 1 is later on improved by LSH, the preprocessing is still preserved.
    \item A2: Thanks for your insightful question. Indeed, Theorem 1 is established in the sense of expectation. But we cannot train Sketch GNNs over different sketches per iteration, since the randomness in the sketches can impede training. Instead, the learnable LSH and sketches are introduced to compensate the fixed number of sketches. Thanks to the gradient signals, we are able to optimize the estimation over a fixed number of sketches directly. Proving an error bound on this learned estimation is much harder, so we relax to randomized sketches in Theorem 1.
    
    \item Q3: After sketching the $n \times n$ adjacency matrix into $c \times c$, the sparsity of the sketch adjacency matrix may increase. The complexity analysis on "Preprocessing" at page 4 probably should not assume the same node degree after sketching.
    \item A3: We did not assume the same sparsity after sketching, but ... (same as R1 A6)
    
    \item Q4: In the improved version of Sketch GNN, the online learning of sketches requires samples of size $|B|$. Yet it is not clear whether $|B|$ needs to depend on graph size $n$ to achieve good error bound. An (informal) discussion would be very helpful.
    \item A4: Because of the ``slow change'' phenomenon of the data-dependent hash tables (left sub-figure of Figure 2), we do not expect large updates of the LSH functions after the early phase of training, and we only need a small subset of nodes whose hash codes are likely outdated to update the LSH functions. As described in part (1) of challenge (2) in Section 4, we select a constant number of hash buckets with the largest gradients and thus $|B|=O(n/c)$ which increases slowly w.r.t. $n$. We will make this point clearer in Section 4.
    
    \item Q5: For experiments, the sizes of the graphs evaluated doesn't seem to be very large (in fact, it belongs to the small- and medium-scale categorization of OGB). More importantly, there seems to be significant accuracy degradation in some cases (Table 2), while the reduction in epoch time is not significant enough (Table 1). In addition, the preprocessing seems to be quite expensive compared with the actual training (Table 1).
    \item A5: We do not agree with these arguments. Firstly, we already test Sketch GNN on \textit{ogbn-product} with 2.45M nodes which is larger than most other graphs. Secondly, with appropriate sketch ratios ($0.2 \sim 0.4$ in Table 3) the performance is always competitive w.r.t. the baselines. It is only when we use a small sketch ratio $0.1$ on a small dataset \textit{ogbn-arxiv} the performance is slightly affected (Table 2), and under this setup only 38.7 MB memory is used (Table 1), far less than the device limit. The reduction in epoch time is considerable (Table 1), since we usually train GNNs for hundreds of epochs. For example, when training for 500 epochs, Sketch GCN will be 181 s faster than full-graph GCN and 85 s faster than GraphSAINT GCN, which are much larger than the pre-processing overhead 27 s. Furthermore, the implementation of sketching (pre-processing) algorithm is not optimized. We expect further speed up if using a sparse FFT algorithm instead of standard FFT. Detailed discussion on the implementation issues will be added to the appendix. 
    
    \item Q6: Secondly, regarding the model design of LSH based Sketch GNN, I have a few questions: The tensor sketch theory relies on data-independent uniformity hashing. It is not clear throughout the paper whether replacing the "vanilla" hashing with LSH would preserve the "data-independent uniformity" property?
    \item A6: Actually without data-independence and uniformity assumptions of the hash functions, similar concentration bounds can still be established (e.g., Theorem 3 in~\citep{weinberger2009feature}), and the corresponding algorithm is known as feature hashing. Feature hashing is essentially identical to count sketch but usually with data-dependent hash functions and mean estimator. Intuitively, it is more challenging to bound the collision errors with randomized hash functions and the median estimator is introduced as it is more robust (Section 3.2 of~\citep{charikar2002finding}). The sketches in Sketch GNN are learned using gradient descent and thus it is hard to obtain an error bound. Thus we build upon count and tensor sketch theory and obtain an error bound when relaxed to randomized hashing. We will discuss about feature hashing and some alternative sketching error bounds (e.g.,~\citep{meister2019tight}) in the appendix.
    
    \item Q7: What are the "parameters" to be learnt for the LSH hash function? From Eq 3, LSH is performed with a random projection matrix $P$. There is no learnable parameter there.
    \item A7: Sorry for the confusion. The projection matrix $P$ in Equation 3 is exactly what we learn in the learnable LSH algorithm as originally proposed in the Section 3.3.1 of~\citep{chen2020mongoose}. The SimHash algorithm described in Section 2 is the standard non-learnable version. We will refine the corresponding part in Section 4.
    
    \item Q8: In the online training of the LSH, how do you obtain the "correct" hash buckets?
    \item A8: This is exactly the second challenge described in Section 4. See Challenge (2) for details and the right sub-figure of Figure 2 for the proof-of-concept experiments.
    
    \item Q9: When you describe LSH as better than the vanilla hash functions, you mentioned that putting similar features in the same bucket reduces the error. Do you implicitly assume that connected nodes in the graph should share similar features? In other words, is sketch-GNN more suitable for graphs of high homophily?
    \item A9: No. LSH does not depend on the topology of the graph, i.e., whether we put two nodes in the same bucket has noting to do with their adjacency. Sketch GNN does not make any assumptions on the homophily and should work equally well for low- and high-homophily graphs.
    
    \item Q10: Thirdly, some description of the related work seems inaccurate. When analyzing the complexity of sampling based methods (e.g., GraphSAGE, GraphSAINT), the authors consider the computation per epoch. I'm not sure if this comparison is fair. In sketch-GNN, one epoch corresponds to one gradient update. However, in those sampling algorithms, one epoch corresponds to many gradient updates (in fact, the number of gradient updates per epoch grows proportionally with the graph size) -- that's why such sampling algorithms appear to be graph size-dependent. I think a more fair comparison would be the total convergence time. Even though it is hard to analyze convergence theoretically, it is still good to clarify this issue in the description of related work and perform some empirical evaluation.
    \item A10: Thanks for the constructive advice. We agree that convergence time could be a better metric to compare Sketch GNN with sampling-based methods. We define the ``convergence time'' as the time for the validation accuracy to reach $99\%$ of the best and find that on \textit{ogbn-arxiv} with sketch dimension or mini-batch size set to $0.1n$ (the setup in Table 1), the convergence time of Sketch GCN is $88\pm8$ s, slightly better than VQ-GNN's ($103\pm11$ s) and GraphSAINT's ($120\pm4$ s). Sketch GCN takes longer number of epochs to converge, but the convergence time is smaller because of the shorter time per epoch. We will add more results and discussions to the appendix.
    
    \item Q11: Lastly, the baseline accuracy listed in Table 2 seems to be lower than those in the original papers / on the public OGB leaderboard.
    \item A11: The listed performance of full-graph GCN, full-graph GraphSAGE, and VQ-GNN in Table 2 and 3 are copied from the OGB leaderboard or original paper. The other results (full-graph GAT, GraphSAINT, Graph Coarsening) could be slightly lower than the elsewhere reported because we only run 500 epochs and repeat the experiment for 5 times. In general these slight differences are within the error bars.
    
    \item Q12: I think this NeurIPS 2021 work is also relevant: Zeng et al. Decoupling the Depth and Scope of Graph Neural Networks. NeurIPS 2021. This related work presents a new sampling algorithm that is much more scalable than GraphSAGE and GraphSAINT.
    \item A12: Thanks for pointing us to this paper. \citet{zeng2021decoupling} propose a novel way to apply GNNs on sampled subgraphs, which decouple the depth and scope of GNNs and lead to better expressivity and scalability. We are interested to add new advances on graph sampling like this to the related work discussion, and consider it as a baseline in the added experiments.
    
\end{itemize}


\section{R5}
\begin{itemize}
    \item Q1: My major concerns are: the sketch compressing operation is not very efficient.
    \item A1: We believe sketching is efficient because: (1) it is an one-time cost, and (2) count and tensor sketch can implemented by sparse matrix multiplication and Fast Fourier Transform, which are supported by highly-optimized libraries like PyTorch. Moreover, the time complexity of count and tensor sketch is better than the other Johnson Lindenstrauss transforms~\citep{meister2019tight}.
    
    \item Q2: The information loss from the compression, especially when being applied to large graphs, is not clear.
    \item A2: In theory, we approximate the original update rule of a GNN With sketching, and the approximation errors are bounded (Theorem 1 and 2). In practice, we can achieve competitive performance on \textit{ogbn-product} with 2.45M nodes with a $0.2$ sketch ratio.
    
    \item Q3: In Line 242, the authors said "If we use the SimHash defined in Eq. (3), an extra $O(ncd)$ computational overhead is introduced." This fact is not intuitive. I hope the authors can explain more in the paper.
    \item A3: SimHash on each feature vector (Equation 3) requires $O(cd)$ time and memory and we have $n$ of them. Hence the total time overhead introduced is $O(ncd)$.
    
    \item Q4: In Table 2, "compression ratio" is reported, while in Table 3, "sketch ratio" is reported. Why there is such inconsistency? Furthermore, I do not find these ratios defined in the paper.
    \item A4: The sketch ratio is defined as $c/n$, the sketch dimension $c$ over the input dimension $n$, in multiple places in the paper (Line 223, Line 415, and the x-axis label of Figure 1). We use ``compression ratio'' in Table 2 because we are comparing with the graph coarsening algorithm, which is a ``pre-compression'' algorithm as ours. Compress ratio, as its name suggests, is the ratio between the uncompressed size and the compressed size. For Sketch GNN, compress ratio is slightly larger than sketch ratio, since there are some memory overheads for learnable LSH. We will add more details on this to Section 7. 
    
    \item Q5: What compression/sketch ratio is used in Table 1? I think that should affect the time complexity for sketch-GNN.
    \item A5: The sketch ratio used in Table 1 is $0.1$ (stated in the caption of Table 1). The training time complexity of Sketch GNN is $O(c)$.
    
    \item Q6: I do not understand why Table 1 and Table 2/3 are examined in different experimental settings. Reporting time complexity alone cannot convince the readers that Sketch-GNN is efficient -- the accuracy should be reported at the same time.
    \item A6: Table 1 is for the comparison of efficiency while Table 2 and 3 are for performance. The performance of the experiments in Table 1 on \textit{ogbn-arxiv} can be found in Table 2 and 3. We will add more performance results on \textit{Reddit} to the appendix.
    
    \item Q7: I am not sure why the current Section 3 and 4 are separated. I think a coherent "Method" section should be much better; it can also reduce a lot of redundant discussions. The current organization further confuses the readers, as I am not sure which part of Section 3 is used in the final version of Sketch-GNN, or they only serve as motivation.
    \item A7: We separate Section 3 (polynomial tensor sketch) and Section 4 (learning sketches with LSH) because (1) they are two main components of Sketch GNN, and (2) they are orthogonal in the sense that the former answers how to compress GNNs and approximate the original update rules with sketches, while the latter addresses how to learn and update the sketches.
    
    \item Q8: The experimental section only takes 1 page including tables. Meanwhile, the paper takes more than 2 pages for all kinds of discussion, which is more than sufficient.
    \item A8: We believe Section 3 and 4 are necessary, since they address two major components of Sketch GNN. We will rewrite Section 4 to improve the presentation. We plan to move Section 5 (generalizing to other GNNs) to the appendix. We will expand Section 7 with the added results and ablation studies.
    
\end{itemize}


%DE-COLORING
\def\colorone{black}
\def\colortwo{black}

==> text/tab_time.tex <==
\begin{table}[!htbp]
\centering
\adjustbox{max width=0.75\textwidth}{%
\begin{threeparttable}
{\renewcommand{\arraystretch}{1.0}%
\begin{tabular}{lcccccc} \toprule
Benchmark                      & \multicolumn{3}{c}{\textit{ogbn-arxiv}} & \multicolumn{3}{c}{\textit{Reddit}}            \\ \arrayrulecolor{black!100} \cmidrule(l){1-1} \cmidrule(lr){2-4} \cmidrule(l){5-7}
Efficiency Measure             & Preprocessing Time  & Epoch Time & Train Memory & Preprocessing Time & Epoch Time & Train Memory \\ \arrayrulecolor{black!50} \cmidrule(l){1-1} \cmidrule(lr){2-4} \cmidrule(l){5-7}
``Full-Graph'' (oracle)        & ---         & 0.49 s     & 983  MB   & ---        & OOM\tnote{1}    & OOM        \\ \arrayrulecolor{black!50} \cmidrule(l){1-1} \cmidrule(lr){2-4} \cmidrule(l){5-7}
GraphSAINT                     & ---         & 0.30 s     & 31.4 MB    & ---        & 2.09 s          & 977 MB     \\ 
VQ-GNN                         & ---         & 0.37 s     & 48.9 MB    & ---        & 2.16 s          & 1281 MB    \\ \arrayrulecolor{black!50} \cmidrule(l){1-1} \cmidrule(lr){2-4} \cmidrule(l){5-7}
Coarsening                     & 358 s       & 0.20 s     & 22.1 MB    & 4123 s     & 1.04 s          & 530 MB     \\ \arrayrulecolor{black!100} \cmidrule(l){1-1} \cmidrule(lr){2-4} \cmidrule(l){5-7}
\textbf{Sketch-GNN (ours)}     & 27 s        & 0.13 s     & 38.7 MB    & 141 s      & 0.81 s          & 748 MB     \\ \arrayrulecolor{black!100} \bottomrule
\end{tabular}}
\appto\TPTnoteSettings{\footnotesize}
\begin{tablenotes}[para]
    \item[1] ``OOM'' refers to ``out of memory''.
\end{tablenotes}
\end{threeparttable}}
\caption{\label{tab:efficiency}Time and memory efficiencies of Sketch-GNN versus other scalable methods.}
\end{table}

